Decomposition Without Regret

Programming languages are embracing both functional and object-oriented paradigms. A key difference between the two paradigms is the way of achieving data abstraction. That is, how to organize data with associated operations. There are important tradeoffs between functional and object-oriented decomposition in terms of extensibility and expressiveness. Unfortunately, programmers are usually forced to select a particular decomposition style in the early stage of programming. Once the wrong design decision has been made, the price for switching to the other decomposition style could be rather high since pervasive manual refactoring is often needed. To address this issue, this paper presents a bidirectional transformation system between functional and object-oriented decomposition. We formalize the core of the system in the FOOD calculus, which captures the essence of functional and object-oriented decomposition. We prove that the transformation preserves the type and semantics of the original program. We further implement FOOD in Scala as a translation tool called Cook and conduct several case studies to demonstrate the applicability and effectiveness of Cook.

==> Dockerfile <==
FROM ubuntu:18.04


RUN apt-get update && \
	apt-get install -y openjdk-8-jdk && \
	apt-get install -y ant && \
	apt-get clean && \
	rm -rf /var/lib/apt/lists/* && \
	rm -rf /var/cache/oracle-jdk8-installer;
	
# Fix certificate issues, found as of 
# https://bugs.launchpad.net/ubuntu/+source/ca-certificates-java/+bug/983302
RUN apt-get update && \
	apt-get install -y ca-certificates-java && \
	apt-get clean && \
	update-ca-certificates -f && \
	rm -rf /var/lib/apt/lists/* && \
	rm -rf /var/cache/oracle-jdk8-installer;

# Setup JAVA_HOME, this is useful for docker commandline
ENV JAVA_HOME /usr/lib/jvm/java-8-openjdk-amd64/
RUN export JAVA_HOME

# Install sbt
SHELL ["/bin/bash", "-c"]
RUN apt update && apt upgrade -y && \
    apt install -y curl && \
    apt install -y zip && \
    apt install -y unzip && \
    curl -s "https://get.sdkman.io" | bash && \
    source "$HOME/.sdkman/bin/sdkman-init.sh" && \
    sdk install sbt


WORKDIR ./FOOD

COPY . . 

==> sections/Background.tex <==
\section{Problem Statement}

